UniPercept: Towards Unified Perceptual-Level Image Understanding across Aesthetics, Quality, Structure, and Texture

Multimodal large language models (MLLMs) have achieved remarkable progress in visual understanding tasks such as visual grounding, segmentation, and captioning. However, their ability to perceive perceptual-level image features remains limited. In this work, we present UniPercept-Bench, a unified framework for perceptual-level image understanding across three key domains: Aesthetics, Quality, Structure and Texture. We establish a hierarchical definition system and construct large-scale datasets to evaluate perceptual-level image understanding. Based on this foundation, we develop a strong baseline UniPercept trained via Domain-Adaptive Pre-Training and Task-Aligned RL, enabling robust generalization across both Visual Rating (VR) and Visual Question Answering (VQA) tasks. UniPercept outperforms existing MLLMs on perceptual-level image understanding and can serve as a plug-and-play reward model for text-to-image generation. This work defines Perceptual-Level Image Understanding in the era of MLLMs and, through the introduction of a comprehensive benchmark together with a strong baseline, provides a solid foundation for advancing perceptual-level multimodal image understanding.

==> unipercept/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> unipercept/sec/main.tex <==

% \vspace{-20pt}
% \twocolumn[{%
% % \maketitle
% \vspace{-40pt}
% \begin{figure}[H]
% \hsize=\textwidth % cvpr 需要
% \centering
% \includegraphics[width=1.5\linewidth]{unipercept/Figures/intro/teaser_v3.9.pdf}
% \vspace{-5pt}
% \caption{\textbf{Overview of UniPercept-Bench.}
% We propose a unified benchmark for perceptual-level image understanding, covering three perceptual domains: Image Aesthetics Assessment (\textbf{IAA}), Image Quality Assessment (\textbf{IQA}), and Image Structure and Texture Assessment (\textbf{ISTA}). 
% Each domain is organized hierarchically into \emph{Domain–Category–Criterion} levels, enabling fine-grained perceptual evaluation. 
% The benchmark contains both Visual Rating (\textbf{VR}) and Visual Question Answering (\textbf{VQA}) tasks, facilitating comprehensive assessment of models’ abilities to understand and reason about perceptual-level image understanding.}
% \label{fig:teaser}
% \end{figure}
% }]

\begin{abstract}
Multimodal large language models (MLLMs) have achieved remarkable progress in visual understanding tasks such as visual grounding, segmentation, and captioning. However, their ability to perceive \textbf{perceptual-level} image features remains limited. In this work, we present \textbf{UniPercept-Bench}, a unified framework for \textit{perceptual-level image understanding} across three key domains: \textbf{Aesthetics}, \textbf{Quality}, \textbf{Structure and Texture}. We establish a hierarchical definition system and construct large-scale datasets to evaluate perceptual-level image understanding. Based on this foundation, we develop a strong baseline \textbf{UniPercept} trained via Domain-Adaptive Pre-Training and Task-Aligned RL, enabling robust generalization across both \textbf{Visual Rating (VR)} and \textbf{Visual Question Answering (VQA)} tasks. UniPercept outperforms existing MLLMs on perceptual-level image understanding and can serve as a \textbf{plug-and-play reward model} for text-to-image generation. This work defines Perceptual-Level Image Understanding in the era of MLLMs and, through the introduction of a comprehensive benchmark together with a strong baseline, provides a solid foundation for advancing perceptual-level multimodal image understanding.
% This work defines \textbf{Perceptual-Level Image Understanding} in the era of MLLMs, and introduces both a comprehensive \textbf{benchmark} and a strong \textbf{baseline} to advance perceptual-level multimodal image understanding.
\end{abstract}



% Recent years have witnessed the rapid advancement of multimodal large language models (MLLMs), which have achieved impressive performance across a variety of vision-language tasks such as segmentation, visual grounding, image captioning and reasoning. These achievements largely stem from their ability to capture and align \textbf{semantic-level representations} between visual and textual modalities. However, while semantic understanding has been extensively explored, the \textbf{perceptual-level comprehension} of images—how humans perceive visual aesthetics, quality, structure, and texture—remains underexplored.

% Human perception of an image involves much more than recognizing objects or scenes; it entails an intricate evaluation of \textit{how} an image looks and feels. Understanding such perceptual-level features is crucial for bridging the gap between machine perception and human visual experience, enabling models to reason about subtle properties such as visual harmony, structural balance, and texture richness. Despite their importance, existing MLLMs often fail to capture these fine-grained perceptual cues, leading to inconsistent or subjective outputs in aesthetic assessment and perceptual reasoning.

% \vspace{-20pt}
% \section{Introduction}
% \label{sec:intro}

% Recent years have witnessed the rapid advancement of multimodal large language models (MLLMs), which have achieved impressive performance across a variety of vision-language tasks such as segmentation, visual grounding, image captioning, visual reasoning and so on~\cite{gpt4, gemini, claude}. These achievements largely stem from their ability to capture and align \textbf{semantic-level representations} between visual and textual modalities~\cite{internvl3,qwen2.5,internvl3-5}. However, while semantic understanding has been extensively explored, the \textbf{perceptual-level comprehension} of images—how humans perceive visual aesthetics, quality, structure, and texture—remains underexplored. As illustrated in Fig.~\ref{fig:task_compare}, \textbf{semantic-level} understanding involves high-level reasoning about objects, relations, and scenes (e.g., captioning or question answering about visible entities), whereas \textbf{perceptual-level} understanding concerns the subjective and fine-grained perception of visual appearance and quality, such as aesthetic appeal, degradation severity, surface texture and so on. 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.4\textwidth]{unipercept/Figures/intro/mission_compare.pdf}
%     \vspace{-10pt}
%     \caption{\textbf{Semantic-level} vs. \textbf{Perceptual-level} Tasks.}
%     % \caption{Comparison of \textbf{Semantic-level} and \textbf{Perceptual-level} image understanding. Semantic-level tasks focus on interpreting object relations and contextual meaning, while perceptual-level tasks emphasize assessing visual appearance and quality.}
%     \label{fig:task_compare}
%     \vspace{-20pt}
% \end{figure}

% Human perception of an image involves much more than recognizing objects or scenes; it entails an intricate evaluation of \textit{how} an image looks and feels. Understanding such perceptual-level features is crucial for bridging the gap between machine perception and human visual experience, enabling models to reason about subtle properties such as visual harmony, structural balance, and texture richness. Despite their importance, existing MLLMs often fail to capture these fine-grained perceptual cues, leading to inconsistent or subjective outputs in aesthetic assessment and perceptual reasoning.


% To address this gap, we propose \textbf{UniPercept}, a unified framework for \textbf{perceptual-level image understanding} across three fundamental perceptual domains: \textbf{I}mage \textbf{A}esthetics \textbf{A}ssessment (\textbf{IAA}), \textbf{I}mage \textbf{Q}uality \textbf{A}ssessment (\textbf{IQA}), and \textbf{I}mage \textbf{S}tructure and \textbf{T}exture \textbf{A}ssessment (\textbf{ISTA}). Our contributions are threefold:
% \begin{itemize}
%     \item \textbf{UniPercept-Bench.} We introduce a comprehensive hierarchical definition of perceptual-level features, consisting of three progressive layers—\textit{Domain, Category, and Criterion}—that systematically describe how perceptual attributes manifest across visual dimensions. Using this taxonomy, we construct \textbf{UniPercept-Bench}, a unified benchmark to quantitatively evaluate perceptual understanding in MLLMs.
    
%     \item \textbf{UniPercept.} We design a domain-adaptive baseline trained through large-scale perceptual-level pre-training and task-aligned reinforcement learning from human feedback. The resulting model demonstrates strong generalization across six perceptual tasks, including both \textbf{V}isual \textbf{R}ating (VR) and \textbf{V}isual \textbf{Q}uestion \textbf{A}
%     nswering (VQA), achieving superior performance over SOTA MLLMs.
    
%     \item \textbf{Practical Applications.} We further validate the application of UniPercept by integrating it as a reward model into existing T2I models, leading to significant and controllable improvements within specified perceptual domains.
% \end{itemize}



% \vspace{-20pt}
\section{Introduction}
\label{sec:intro}

Recent years have witnessed the rapid advancement of multimodal large language models (MLLMs), which now achieve impressive performance across a variety of vision–language tasks including segmentation, visual grounding, image captioning, and visual reasoning~\cite{gpt4, gemini, claude}. These advancements are largely driven by their strong capability to learn and align semantic-level representations, allowing models to identify objects and scenes, capture their relationships and perform visual reasoning~\cite{internvl3,qwen2.5,internvl3-5}.

However, despite extensive progress on semantic understanding, the perceptual-level comprehension of images—how humans perceive aesthetics, quality, structure, and texture—remains substantially underexplored. As illustrated in Fig.~\ref{fig:task_compare}, \textbf{semantic-level} tasks focus on high-level interpretation of visual entities (e.g., object attributes or contextual reasoning), whereas \textbf{perceptual-level} tasks require assessing fine-grained, low-level visual appearance, such as aesthetic harmony, degradation severity, structural regularity, or surface texture. These perceptual attributes are inherently subtle, often subjective, and closely tied to human visual experience, making them fundamentally different from typical semantic-level tasks.

% Human visual perception involves much more than object recognition: it includes nuanced judgments about \textit{how} an image looks and feels. Such perceptual cues play a crucial role in many downstream applications (e.g., content creation, image enhancement, and generative model alignment). Nevertheless, current MLLMs often struggle with these aspects, producing unstable or inconsistent predictions when evaluating aesthetic quality, perceptual degradation, or structural coherence. This gap highlights the need for a unified framework that can \textit{explicitly define, evaluate, and improve} perceptual-level understanding in MLLMs.

Human visual perception involves much more than object recognition: it includes nuanced judgments about \textit{how} an image looks and feels. Such perceptual cues play a crucial role in many downstream applications (e.g., content creation, image enhancement, and generative model alignment). Nevertheless, current MLLMs often struggle with these aspects, producing unstable or inconsistent predictions when evaluating aesthetic quality, perceptual degradation, or structural coherence. This gap highlights the need for a unified framework that can \textit{explicitly define, evaluate, and improve} perceptual-level understanding in MLLMs, as perceptual attributes remain far less standardized and less explored than semantic ones. Addressing this missing layer is essential for building models that align more closely with human judgments, thereby achieving higher visual quality.

\begin{figure}[htbp]
    % \vspace{-10pt}
    \centering
    \includegraphics[width=0.45\textwidth]{unipercept/Figures/intro/mission_compare_v3.pdf}
    \vspace{-5pt}
    \caption{\textbf{Semantic-level} vs. \textbf{Perceptual-level} understanding.}
    \label{fig:task_compare}
    % \vspace{-10pt}
\end{figure}

% \textbf{I}mage \textbf{A}esthetics \textbf{A}ssessment (\textbf{IAA}), \textbf{I}mage \textbf{Q}uality \textbf{A}ssessment (\textbf{IQA}), and \textbf{I}mage \textbf{S}tructure and \textbf{T}exture \textbf{A}ssessment (\textbf{ISTA})

To bridge this gap, we propose \textbf{UniPercept}, the first unified framework for \textbf{perceptual-level image understanding} across three core domains: Image Aesthetics Assessment (\textbf{IAA}), Image Quality Assessment (\textbf{IQA}), and Image Structure and Texture Assessment (\textbf{ISTA}). Our contributions are summarized as follows:

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{unipercept/Figures/benchmark/qa_example_v1_2.pdf}
    \vspace{-5pt}
    \caption{\textbf{Representative QA examples in UniPercept-Bench.}
Questions follow a three-level hierarchy of \textit{Domain–Category–Criterion}, defining perceptual scope, specific visual aspects, and fine-grained criteria for constructing diverse, perception-oriented VQA tasks.}
    \label{fig:qa_example}
    % \vspace{-20pt}
\end{figure*}


\begin{itemize}
    \item \textbf{UniPercept-Bench.}  
    We establish a comprehensive hierarchical taxonomy of perceptual attributes, consisting of three progressive layers: \textit{Domain–Category–Criterion}. Building upon this taxonomy, we construct UniPercept-Bench, a systematically designed benchmark for evaluating perceptual-level image understanding in MLLMs. The benchmark covers fine-grained perceptual attributes and supports both Visual Rating (\textbf{VR}) and Visual Question Answering (\
    \textbf{VQA}) tasks for unified perceptual-level image understanding.

    \item \textbf{UniPercept.}  
    We develop \textbf{UniPercept} as a strong baseline MLLM through large-scale Domain-Adaptive Pre-Training and task-aligned reinforcement learning. Without relying on additional human feedback, the model learns to reliably assess perceptual attributes across diverse visual domains. UniPercept demonstrates strong generalization across both \textbf{VR} and \textbf{VQA} tasks, and achieves consistent gains in all three perceptual domains (\textbf{IAA}, \textbf{IQA}, and \textbf{ISTA}), substantially outperforming state-of-the-art generalized and specialized MLLMs.
    % UniPercept demonstrates strong generalization across two perceptual tasks, covering both \textbf{VR} and \textbf{VQA}, and achieves consistent gains across all three perceptual domains (\textbf{IAA}, \textbf{IQA}, and \textbf{ISTA}), substantially outperforming state-of-the-art MLLMs.
    % UniPercept demonstrates strong generalization across two perceptual tasks—spanning both \textbf{VR} and \textbf{VQA}—and achieves consistent gains across all three perceptual domains: \textbf{IAA}, \textbf{IQA}, and \textbf{ISTA}, substantially outperforming state-of-the-art MLLMs.
    % UniPercept demonstrates strong generalization across six perceptual tasks and substantially outperforms state-of-the-art MLLMs.

    % \item \textbf{Application.}  
    % We further showcase the utility of UniPercept by integrating it as a plug-and-play reward model into text-to-image (T2I) model post training.~\cite{liu2025flowgrpotrainingflowmatching} This integration yields controllable improvements in specific perceptual dimensions, demonstrating the practical value of perceptual-level modeling for generative image applications.
    % \item \textbf{Practical Application for T2I Models.}  
    % We demonstrate the practical value of UniPercept by using it as a \textbf{plug-and-play reward model} in the post-training fine-tuning stage of text-to-image (T2I) models~\cite{liu2025flowgrpotrainingflowmatching}.  
    % By directly optimizing perceptual-level signals (e.g. aesthetic quality, structural richness, scene diversity) this integration leads to clear and controllable improvements in the perceptual quality of generated images.
    \item \textbf{Applications of UniPercept.}
UniPercept serves as a strong plug-and-play \textbf{reward model} for post-training T2I models~\cite{liu2025flowgrpotrainingflowmatching}, enabling direct optimization of perceptual-level signals such as aesthetic quality, structural richness, and scene diversity. This integration yields clear and controllable improvements in the perceptual quality of generated images.
Beyond reward optimization, UniPercept also functions as a unified perceptual metric for evaluating images and as a tool for characterizing perceptual distributions in large-scale datasets.
    
\end{itemize}


% \vspace{-10pt}
\section{Related Works}
\label{sec:related_work}

\subsection{MLLM Benchmark}
\label{sec:mllm_benchmark}
% MLLM benchmark的发展历程和现状，主要是说明：
% 1.这些benchmark都在尝试提出什么类型的问题，尝试评估模型的什么方面能力
% 2.说明这些benchmark的共性：其中问题都聚焦于语义级别理解层面
% 参考：mmmu, mmmu-pro, mega-bench, mmstar, mmbench, mathvista, ocrbench
% 更多可以参考：https://huggingface.co/spaces/opencompass/open_vlm_leaderboard

With the rapid development of MLLMs, evaluating their performance has gone far beyond simple semantic understanding tasks such as image recognition or segmentation. In recent years, researchers have begun to assess whether a model can achieve a deeper level of understanding and reasoning about visual content.

For instance, MMMU~\cite{mmmu} focuses on university-level exam questions across diverse disciplines, while MMMU-Pro~\cite{mmmu-pro} extends this idea with more complex, cross-domain reasoning challenges. MEGA-Bench~\cite{mega-bench} emphasizes large-scale multimodal comprehension and knowledge integration, and MMStar~\cite{mm-star} targets general reasoning and factual understanding in visual contexts. MMBench~\cite{mmbench} evaluates comprehensive perception and reasoning across everyday images, MathVista~\cite{mathvista} centers on mathematical and geometric reasoning within visual scenes, and OCRBench~\cite{ocrbench} specifically tests a model’s capability to recognize and interpret text embedded in images.

% However, these benchmarks mainly transform visual information into textual representations before reasoning, focusing more on language-based inference rather than pure visual understanding. In contrast, our proposed UniPercept-Bench evaluates a model’s ability to perceptual-level intrinsic visual properties such as technical execution, distortion location, material representation and so on, thereby bridging the gap between perceptual and semantic-level understanding.

However, these benchmarks rely on converting visual content into text representations before reasoning, emphasizing language-based inference over genuine visual understanding. In contrast, UniPercept-Bench directly evaluates perceptual-level visual properties—such as technical execution, distortion location, and material depiction—bridging the gap between perceptual and semantic understanding.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{unipercept/Figures/benchmark/bench_pipeline_v3.5.pdf}
    \vspace{-5pt}
    \caption{\textbf{Constuction pipeline of UniPercept-Bench.} A three-stage process initial QA generation, reject sampling, and human refinement to produce high-quality perceptual-level QA pairs across aesthetics, quality, structure, and texture. }
    \label{fig:benchmark_pipeline}
    % \vspace{-15pt}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{unipercept/Figures/benchmark/table_v6.png}
    \vspace{-5pt}
    \caption{\textbf{Distribution of UniPercept-Bench} across (a) Domain, (b) Category, and (c) Criterion. Zoom in for best view.}
    \label{fig:benchmark_distribution}
    % \vspace{-20pt}
\end{figure}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{unipercept/Figures/benchmark/table—V4.png}
%     \vspace{-20pt}
%     \caption{\textbf{Distribution of UniPercept-Bench} across (a) QA Template, (b) Domain, (c) Category, and (d) Criterion. Zoom in for best view.}
%     \label{fig:benchmark_distribution}
%     \vspace{-20pt}
% \end{figure*}

% \vspace{-5pt}
\subsection{Image Assessment}
\label{sec:image_assessment}
% IAA IQA ISTA研究发展历程和现状
% IAA：Q-align，UNIAA，ArtiMuse，Aes-R1
% IQA：MUSIQ，DepictQA，DepictQA-Wild，DeQA，Q-insight
% ISTA：几乎空白
% benchmark一直不成体系，且其中很多benchmark用现在的mllm模型去测试已经很轻易能达到很高的准确率，一定程度上失去意义：q-bench，q-bench++，AesBench

% For low-level vision tasks, we categorize evaluation into three main types: \textbf{I}mage \textbf{A}esthetics \textbf{A}ssessment (\textbf{IAA}), \textbf{I}mage \textbf{Q}uality \textbf{A}ssessment (\textbf{IQA}), and \textbf{I}mage \textbf{S}tructure and \textbf{T}exture \textbf{A}ssessment (\textbf{ISTA}).
% At present, many benchmarks and methods have been developed for the first two categories. For example, IAA includes Q-align~\cite{qalign}, UNIAA~\cite{Uniaa} and ArtiMuse~\cite{artimuse}, while IQA includes MUSIQ~\cite{Musiq}, DepictQA~\cite{depictqa_v1}, DepictQA-Wild~\cite{depictqa_v2}, DeQA~\cite{deqa_score}, and Q-Insight~\cite{Q-insight}. However, there is still no dedicated dataset for ISTA, leaving sthe evaluation of texture perception largely unexplored.

For perceptual-level image assessment, prior research has primarily focused on two major areas: 
Image Aesthetics Assessment (IAA) and 
Image Quality Assessment (IQA). 
Extensive benchmarks and methods have been developed for these two categories—for example, 
Q-Align~\cite{qalign}, UNIAA~\cite{Uniaa}, and ArtiMuse~\cite{artimuse} for IAA, and 
MUSIQ~\cite{Musiq}, DepictQA~\cite{depictqa_v1,depictqa_v2}, DeQA~\cite{deqa_score}, and Q-Insight~\cite{Q-insight} for IQA. In contrast, another crucial perceptual dimension—Image Structure and Texture Assessment (\textbf{ISTA})—has received far less systematic attention. 
Although a few prior works~\cite{dtd,fmd} touch upon aspects of structural or textural perception, they do not provide a unified or comprehensive definition of ISTA, leaving this important component of perceptual-level understanding still insufficiently explored.

In addition, most existing datasets focus on a single aspect such as numerical scoring or question answering, without providing a comprehensive and multi-dimensional evaluation framework. As multimodal large models continue to improve, many existing models have already achieved very high accuracy on prior benchmarks~\cite{Aesbench,Q-bench,Q-bench++}, reducing the ability of these benchmarks to effectively distinguish stronger models. In contrast, our UniPercept-Bench addresses these limitations by covering multiple perceptual dimensions, offering diverse and detailed evaluation data, and presenting a more comprehensive challenge for MLLMs.



% Benchmark
% \vspace{-10pt}
\section{UniPercept-Bench}
\label{sec:benchmark}

% \vspace{-10pt}
\subsection{Definition}
\label{sec:definition}
% \vspace{-10pt}

% UniPercept-Bench targets \textbf{perceptual-level} image understanding across three domains—\textbf{I}mage \textbf{A}esthetics \textbf{A}ssessment (\textbf{IAA}), \textbf{I}mage \textbf{Q}uality \textbf{A}ssessment (\textbf{IQA}), and \textbf{I}mage \textbf{S}tructure and \textbf{T}exture \textbf{A}ssessment (\textbf{ISTA}).
% While IAA and IQA have been extensively explored in prior studies such as Q-Align~\cite{qalign}, the DepictQA series~\cite{depictqa_v1,depictqa_v2,deqa_score}, and ArtiMuse~\cite{artimuse}, we further consolidate and refine their definitions for unified perceptual evaluation.
% In contrast, ISTA remains largely underexplored despite its central role in human perception. Motivated by advances in image generation and low-level vision, we introduce the first systematic and operational definition of ISTA, focusing on the assessment of structural integrity, texture realism, and material fidelity—crucial aspects for aligning machine perception with human visual sensitivity.

% We adopt a three-tier taxonomy: Domain/Category/Criterion, as shown in Fig.1. The domain specifies scope, categories partition the space into discriminable subtypes, and criterion provide actionable, testable rules. For each criterion of IAA and IQA, we consolidate widely accepted expert-level definitions. For ISTA, we conduct focused discussions with practitioners possessing relevant professional experience to establish precise, consensus-driven definitions.

% Building on this taxonomy, UniPercept-Bench offers two task forms with objective targets:
% \begin{itemize}
% \item \textbf{Visual Rating (VR)}: Models output a continuous score for comprehensive assessment of each domain—IAA (aesthetics), IQA (quality), and ISTA (structure and texture richness)—evaluating calibrated, perceptually aligned quantitative judgments.
% \item \textbf{Visual Question Answering (VQA)}: Question sets are designed at the Domain/Category/Criterion levels with diverse foci and formats, assessing perceptual-level understanding, image–text grounding, and explanatory competence.
% \end{itemize}
% Together, VR and VQA constitute a unified evaluation framework coupling quantitative judgment with explanatory consistency.

As shown in Fig.~\ref{fig:teaser}, UniPercept-Bench targets \textbf{perceptual-level} image understanding across Image Aesthetics Assessment (IAA), Image Quality Assessment (IQA), and Image Structure and Texture Assessment (ISTA). \textbf{IAA} focuses on the \textit{perceived aesthetic attributes} of an image, such as composition, style, emotion, and overall visual appeal. \textbf{IQA} targets the \textit{perceived fidelity and degradation factors}, including noise, blur, compression artifacts, and overall distortion levels. \textbf{ISTA} evaluates the \textit{structural and textural characteristics} of a scene, emphasizing geometry, material properties, and local detail richness. Although all three domains assess images, the tasks focus on fundamentally \textbf{different aspects}. For example, a high-quality image may not possess strong aesthetic value, while an aesthetically pleasing image may contain only simple or sparse textures.

While IAA and IQA have been widely studied in prior works such as Q-Align~\cite{qalign}, the DepictQA series~\cite{depictqa_v1,depictqa_v2,deqa_score}, and ArtiMuse~\cite{artimuse}, \textbf{ISTA} remains largely unexplored, with little prior effort to systematically define or evaluate it. Inspired by recent advances in image generation and low-level vision~\cite{flux,wu2025qwenimagetechnicalreport,supir}, we reorganize and unify the existing definition systems for IAA and IQA, and propose the \textbf{first} systematic, operational definition of ISTA. Together, these three domains form a coherent perceptual-level framework that enables comprehensive and fine-grained assessment of IAA, IQA ans ISTA cues aligned with human perception. More details are provided in the Appendix.

% While IAA and IQA have been widely studied in works such as Q-Align~\cite{qalign}, the DepictQA series~\cite{depictqa_v1,depictqa_v2,deqa_score}, and ArtiMuse~\cite{artimuse}, \textbf{ISTA} remains largely unexplored, with little prior work systematically defining or evaluating. Inspired by recent progress in image generation and low-level vision~\cite{flux,wu2025qwenimagetechnicalreport,supir}, we introduce the first systematic and operational definition of ISTA, enabling fine-grained assessment of structure- and texture-related cues that more closely align machine perception with human perceptual judgments.

% While IAA and IQA have been extensively explored in prior works such as Q-Align~\cite{qalign}, the DepictQA series~\cite{depictqa_v1,depictqa_v2,deqa_score}, and ArtiMuse~\cite{artimuse}, we further standardize and unify their definitions under a coherent perceptual framework.
% In contrast, \textbf{ISTA}—a domain central to human perception yet rarely studied—focuses on the assessment of structural integrity, texture comprehensiveness and so on.
% Motivated by advances in image generation and low-level vision, we establish the first systematic and operational definition of ISTA, enabling fine-grained evaluation of structure- and texture-related perceptual cues that bridge machine and human perception.

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{unipercept/Figures/benchmark/training_pipeline_v2.pdf}
    \vspace{-5pt}
    \caption{\textbf{Training pipeline of UniPercept.} 
A two-stage framework combining domain-adaptive pre-training for perceptual understanding and task-aligned RL to jointly optimize Visual Rating and Visual Question Answering.}
    \label{fig:training_pipeline}
    % \vspace{-20pt}
\end{figure*}

% We organize UniPercept-Bench using a three-tier taxonomy of \textit{Domain–Category–Criterion}.
% For IAA and IQA, we consolidate expert-agreed definitions from prior literature.
% For ISTA, we conduct structured interviews with domain practitioners to derive precise, consensus-driven perceptual criteria. Building on this taxonomy, UniPercept-Bench introduces two complementary task forms:

% % \noindent\textbf{Visual Rating (VR).} Models output a continuous score representing perceptual alignment across IAA (aesthetics quality), IQA (image quality), and ISTA (structure and texture richness). This task evaluates calibrated, quantitative perception. For ISTA, we first perform structured annotations following the definition framework of UniPercept-Bench to characterize scene composition, geometric layout, and material representation. 
% % The resulting scores constitute the ISTA Rating dataset (\textit{ISTA-10K}), from which 970 samples were randomly selected as the test set.

% \noindent\textbf{Visual Rating (VR).} 
% Models output a continuous score representing perceptual alignment across IAA (aesthetics quality) and IQA (image quality), serving as a quantitative measure of perceptual understanding. 
% We additionally define the \textbf{ISTA Rating} task to evaluate \textit{structure and texture richness}, where a higher score indicates a scene with more complex geometry and richer textures. 
% Following the definition framework of UniPercept-Bench, we design a scoring method that computes the ISTA score by aggregating and weighting the counts of structured attributes extracted from each image, as detailed in the Appendix.

% \noindent\textbf{Visual Question Answering (VQA).} Question sets are constructed at the \textit{Domain–Category–Criterion} levels to assess perceptual-level understanding and reasoning.





% % Together, VR and VQA form a unified evaluation protocol that jointly measures \textbf{quantitative judgment} and \textbf{explanatory consistency}, advancing comprehensive perceptual-level understanding.

% Together, VR and VQA form a unified evaluation protocol that jointly measures \textbf{quantitative judgment} and \textbf{explanatory consistency}, advancing comprehensive perceptual-level understanding, as illustrated in Fig.~\ref{fig:qa_example}.

% \subsection{Benchmark Construction}
% \label{sec:benchmark_construction}
% We follow prior works~\cite{artimuse,vgr} and build a complete, scalable pipeline (as shown in Fig.~\ref{fig:benchmark_pipeline}) to generate high-quality QA pairs grounded in our definition taxonomy.

% \noindent\textbf{Initial QA Generation.}
% We sample, filter, and curate images across three dimensions (IAA, IQA and ISTA) from multiple datasets to ensure both source diversity and coverage of diverse phenomena. Concretely, we balance aesthetic quality for IAA, degradation levels for IQA, and scene granularity for ISTA (local-, object-, and scene-level).
% For IAA and IQA, we rely on expert-annotated datasets~\cite{artimuse,depictqa_v2,q-ground} and adopt the original labels as the professional evaluation. For ISTA, we design prompts containing detailed priors derived from our taxonomy; GPT-4o~\cite{gpt4} is used to ingest these priors and produce structured annotations, which are subsequently filtered and treated as the professional evaluation.
% Given each image and its annotations, we select the corresponding \textit{Domain–Category–Criterion} definitions from the taxonomy and a matched question template from the template bank. These inputs are fed to the Generator MLLM (GPT-4o) to produce the initial QA pairs. To improve quality and enable downstream verification, the generator outputs the question, answer, and a concise chain-of-thought rationale.



% \noindent\textbf{Reject Sampling.}
% We invoke a heterogeneous Judger MLLM to evaluate each initial sample using the question, answer, and rationale. The judge scores four criteria---\textbf{Answer Validity}, \textbf{Question Validity}, \textbf{Reasoning Validity}, and \textbf{Criterion Relevance}---on a five-point scale: bad/poor/fair/good/excellent. A sample is retained only if it achieves \textbf{good} or \textbf{excellent} on all criteria. This reject-sampling step filters out approximately 40\% data.



% \noindent\textbf{Human Refinement.}
% Finally, trained volunteers with backgrounds in Image Assessment conduct a human-centric review. They remove items that do not align with human reasoning habits and lightly edit borderline cases to meet our standards.
% After this refinement, we obtain high-quality QA pairs that are both taxonomically aligned and consistent with human perception, which constitute the data units of UniPercept.

% \vspace{-5pt}
\subsection{Benchmark Construction}
\label{sec:benchmark_construction}

% We establish a complete and scalable pipeline for constructing UniPercept-Bench, as illustrated in Fig.~\ref{fig:benchmark_pipeline}. 
% The process integrates structured priors, multimodal generation, automatic validation, and human refinement to produce high-quality, taxonomy-aligned QA pairs.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{unipercept/Figures/benchmark/qa_example_v1_1.pdf}
%     \vspace{-10pt}
%     \caption{\textbf{Representative QA examples in UniPercept-Bench.}
% Questions follow a three-level hierarchy of \textit{Domain–Category–Criterion}, defining perceptual scope, specific visual aspects, and fine-grained criteria for constructing diverse, perception-oriented VQA tasks.}
%     \label{fig:qa_example}
%     \vspace{-20pt}
% \end{figure*}

We organize UniPercept-Bench using a three-tier taxonomy of \textit{Domain–Category–Criterion}.
For IAA and IQA, we consolidate expert-agreed definitions from prior literature.
For ISTA, we conduct structured interviews with domain practitioners to derive precise, consensus-driven perceptual criteria. Building on this taxonomy, UniPercept-Bench introduces two complementary task forms:

% \noindent\textbf{Visual Rating (VR).} Models output a continuous score representing perceptual alignment across IAA (aesthetics quality), IQA (image quality), and ISTA (structure and texture richness). This task evaluates calibrated, quantitative perception. For ISTA, we first perform structured annotations following the definition framework of UniPercept-Bench to characterize scene composition, geometric layout, and material representation. 
% The resulting scores constitute the ISTA Rating dataset (\textit{ISTA-10K}), from which 970 samples were randomly selected as the test set.

\noindent\textbf{Visual Rating (VR).} 
Models output a continuous score representing perceptual alignment across IAA (aesthetics quality) and IQA (image quality), serving as a quantitative measure of perceptual understanding. 
We additionally define the \textbf{ISTA Rating} task to evaluate \textit{structure and texture richness}, where a higher score indicates a scene with more complex geometry and richer textures. 
Following the definition framework of UniPercept-Bench, we design a scoring method that computes the ISTA score by aggregating and weighting the counts of structured attributes extracted from each image, as detailed in the Appendix.

\noindent\textbf{Visual Question Answering (VQA).} Question sets are constructed at the \textit{Domain–Category–Criterion} levels to assess perceptual-level understanding and reasoning. Together, VR and VQA form a unified evaluation protocol that jointly measures \textbf{quantitative judgment} and \textbf{explanatory consistency}, advancing comprehensive perceptual-level understanding, as illustrated in Fig.~\ref{fig:qa_example}.





% Together, VR and VQA form a unified evaluation protocol that jointly measures \textbf{quantitative judgment} and \textbf{explanatory consistency}, advancing comprehensive perceptual-level understanding.

% Together, VR and VQA form a unified evaluation protocol that jointly measures \textbf{quantitative judgment} and \textbf{explanatory consistency}, advancing comprehensive perceptual-level understanding, as illustrated in Fig.~\ref{fig:qa_example}.


\noindent\textbf{Initial QA Generation.}
As illustrated in Fig.~\ref{fig:benchmark_pipeline}, We begin by collecting images from three perceptual dimensions to ensure diversity across aesthetic quality, distortion severity, and structural complexity. For IAA and IQA, we adopt expert-annotated datasets~\cite{artimuse,depictqa_v2,q-ground} as professional evaluations. 
For ISTA, we introduce structured annotations guided by UniPercept-Bench’s taxonomy, describing scene composition, geometric layout, and material representation.
These annotations are paired with predefined \textit{Domain–Category–Criterion} definitions and matched templates from a curated \textit{Question Template Bank}. The \textit{Generator MLLM} (GPT-4o~\cite{gpt4}) combines the image, annotation, and template to produce candidate QA pairs along with brief reasoning rationales.
% The \textit{Generator MLLM} (GPT-4o~\cite{gpt4}) integrates these components—image, annotation, and template—to generate candidate QA pairs, each accompanied by a concise reasoning rationale.

\noindent\textbf{Reject Sampling.} A heterogeneous \textit{Judger MLLM} (Qwen-2.5-VL-78B-Instruct~\cite{qwen2.5}) evaluates each QA pair on \textbf{Question Validity}, \textbf{Answer Validity}, \textbf{Reasoning Validity}, and \textbf{Criterion Relevance}using a five-point scale. Only samples rated \textit{good} or above on all aspects are retained, removing about 40\% of candidates.

% \noindent\textbf{Reject Sampling.} The heterogeneous \textit{Judger MLLM} (Qwen-2.5-VL-78B-Instruct~\cite{qwen2.5}) then evaluates each QA pair across four aspects—\textbf{Question Validity}, \textbf{Answer Validity}, \textbf{Reasoning Validity}, and \textbf{Criterion Relevance}.
% Each is scored on a five-point scale (\textit{bad–poor–fair–good–excellent}), and only samples rated \textit{good} or above in all aspects are retained, filtering out roughly 40\% of candidates.
% Each generated QA pair is then automatically reviewed by a heterogeneous \textit{Judger MLLM} (Qwen-2.5-VL-78B-Instruct~\cite{qwen2.5}), which assesses four dimensions: \textbf{Question Validity}, \textbf{Answer Validity}, \textbf{Reasoning Validity}, and \textbf{Criterion Relevance}. 
% Each dimension is rated on a five-point scale (\textit{bad–poor–fair–good–excellent}), and only samples rated \textit{good} or above in all dimensions are retained. 
% This reject-sampling stage removes approximately 40\% samples.


\noindent\textbf{Human Refinement.}
Finally, trained volunteers with expertise in Image Assessment conduct manual validation to ensure alignment with human reasoning and perception. 
Borderline cases are revised for clarity and consistency, while invalid samples are removed. 
The resulting dataset consists of high-quality QA pairs that are both perceptually grounded and semantically coherent.

% \subsection{Comparison With Other Benchmarks}
% \label{sec:comparion_with_other_benchmark}

% Baseline
% \vspace{-10pt}
\section{UniPercept}
\label{sec:baseline}

\subsection{Domain-Adaptive Pre-Training}
\label{sec:pretrain}

We aim to train a model with perceptual-level understanding ability across Aesthetics, Quality, Structure, and Texture. To endow the model with a foundational capability for perceptual-level image understanding, we first conduct a \textbf{Domain-Adaptive Pre-Training} stage. Specifically, we select and process large-scale existing datasets, resulting in two types of pre-training data as follows:

% \noindent\textbf{Text-based QA pairs.} We construct extensive QA pairs for IAA, IQA, and ISTA tasks. In particular, for ISTA, we further introduce structured-output QA pairs, as illustrated in Fig.~\ref{fig:training_pipeline}, enabling the model to learn fine-grained structural reasoning.

\noindent\textbf{Text-based QA pairs.} We construct large-scale QA pairs for IAA, IQA, and ISTA. For ISTA, we additionally design structured-output QA pairs (Fig.~\ref{fig:training_pipeline}) to support fine-grained structural reasoning.

\noindent\textbf{VR-based QA pairs.} We additionally incorporate VR data for IAA, IQA, and ISTA, also visualized in Fig.~\ref{fig:training_pipeline}, which allows the model to directly associate perceptual-level attributes with quantitative ratings.

In total, the dataset in domain-adaptive pre-training contains approximately \textbf{800K} samples. Through Domain-Adaptive Pre-Training, the model acquires the essential capability to handle diverse perceptual-level image understanding tasks across different domains.

% \vspace{-5pt}
\subsection{Task-Aligned RL for VR \& VQA}
\label{sec:rl}
% \vspace{-5pt}

% 如表格1，2，3所示，
\begin{table*}[t!]
\centering
\small
\caption{\textbf{Performance comparison of different models on UniPercept-Bench-VR.}
The best results are highlighted with \legendlabel{100}{dark blue} cells, and the second-best results with \legendlabel{40}{light blue} cells.
Models with * indicate those retrained on ArtiMuse-10K, KonIQ-10K, and ISTA-10K. "-/-" denotes cases where the model refuse to respond or fail to provide valid answers due to functional limitations. Metrics: SRCC/PLCC.}
% \vspace{-10pt}
\resizebox{\textwidth}{!}{
\begin{threeparttable}[t]
\renewcommand{\arraystretch}{0.9} % 调整行距，默认1.0，数值越小行距越紧凑
\begin{tabular}{l|ccccc|ccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{5}{c|}{\textbf{VR - IAA}} &
\multicolumn{5}{c|}{\textbf{VR - IQA}} &
\multicolumn{1}{c}{\textbf{VR - ISTA}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-12}
 & ArtiMuse-10K~\cite{artimuse} & AVA~\cite{ava} & TAD66K~\cite{tad66k}& FLICKR-AES~\cite{flickr} & \textbf{Avg.} &
 KonIQ-10K~\cite{koniq} & SPAQ~\cite{spaq} & KADID~\cite{kadid10k} & PIPAL~\cite{pipal}& \textbf{Avg.} &
 ISTA-10K \\
\midrule

\multicolumn{1}{l}{\textit{\textbf{Proprietary Models}}} & \multicolumn{11}{c}{\textit{\textcolor{myblue}{\textbf{Large-scale Pretraining, Cross domain testing}}}} \\
GPT-4o~\cite{gpt4}  &
0.333/0.276 & \bluecellnp{70}0.509/0.485 & 0.278/0.282 & 0.605/0.597 & \bluecellnp{70}0.431/0.410 &
0.695/0.744 & 0.874/0.881 & 0.677/0.646 & 0.325/0.349 & 0.643/0.655 & -0.003/0.116 \\
Llama-4-Scout~\cite{meta_llama4_scout_2025}  &
0.204/0.147 & 0.345/0.329 & 0.236/0.210 & 0.548/0.506 & 0.333/0.298 &
0.503/0.653 & -0.041/0.007 & -0.099/-0.004 & -0.007/0.023 & 0.089/0.170 & -0.025/0.047 \\
Gemini-2.5-pro~\cite{gemini}  &
0.187/0.035 & 0.248/0.100 & 0.143/0.037 & 0.357/0.206 & 0.234/0.095 &
0.582/0.316 & 0.087/0.212 & 0.436/0.274 & 0.225/-0.019 & 0.333/0.196 & -0.230/-0.118 \\
Claude-Sonnet-4.5~\cite{claude}  &
0.041/0.027 & 0.003/0.013 & 0.040/0.047 & 0.037/0.049 & 0.030/0.034 &
-0.037/-0.043 & 0.036/0.085 & 0.223/0.273 & -0.131/-0.088 & 0.023/0.057 & 0.125/0.089 \\
Claude-Sonnet-4.5-Think~\cite{claude}  &
0.066/0.103 & 0.018/0.019 & 0.026/0.039 & -/- & 0.037/0.054 &
-/- & -/- & -/- & -/- & -/- & -/- \\

\midrule
\multicolumn{1}{l}{\textit{\textbf{Open-Source Models}}} & \multicolumn{11}{c}{\textit{\textcolor{myblue}{\textbf{Large-scale Pretraining, Cross domain testing}}}} \\
LLaVA-OneVision-1.5-Instruct-8B~\cite{LLaVA-OneVision-1.5}  &
0.274/0.212 & 0.381/0.378 & 0.213/0.224 & 0.586/0.541 & 0.364/0.339 &
0.639/0.744 & -/- & 0.505/0.534 & 0.417/0.407 & 0.520/0.562 & -0.094/0.027 \\
GLM-4.5-V-106BA12B~\cite{glm}  &
0.346/0.249 & 0.464/0.420 & \bluecellnp{70}0.289/0.278 & \bluecellnp{70}0.651/0.597 & 0.438/0.386 &
0.721/0.765 & -0.040/-0.038 & -0.142/-0.128 & 0.013/0.020 & 0.138/0.155 & 0.083/0.117 \\
InternVL3-8B~\cite{internvl3}  &
0.245/0.211 & 0.372/0.344 & 0.205/0.191 & 0.547/0.476 & 0.342/0.306 &
0.574/0.646 & 0.828/0.800 & 0.496/0.475 & 0.435/0.459 & 0.583/0.595 & -0.127/0.046 \\
InternVL3-78B~\cite{internvl3}  &
0.223/0.206 & 0.385/0.344 & 0.221/0.220 & 0.518/0.433 & 0.337/0.301 &
0.635/0.676 & 0.849/0.852 & 0.579/0.553 & 0.415/0.457 & 0.619/0.634 & -/- \\
InternVL3.5-8B~\cite{internvl3-5}  &
0.135/0.104 & 0.308/0.295 & 0.180/0.182 & 0.519/0.448 & 0.286/0.257 &
0.663/0.660 & 0.783/0.777 & 0.541/0.478 & 0.351/0.386 & 0.585/0.575 & -0.096/-0.025 \\
InternVL3.5-38B~\cite{internvl3-5}  &
0.219/0.175 & 0.359/0.357 & 0.201/0.208 & 0.559/0.529 & 0.334/0.317 &
0.578/0.652 & 0.840/0.831 & 0.568/0.537 & 0.448/0.457 & 0.608/0.619 & \bluecellnp{70}0.262/0.345 \\
QwenVL-2.5-Instruct-7B~\cite{qwen2.5}  &
0.223/0.143 & 0.359/0.324 & 0.208/0.195 & 0.588/0.520 & 0.345/0.296 &
0.708/0.762 & -/- & 0.521/0.517 & 0.350/0.361 & 0.526/0.547 & -0.046/0.076 \\
QwenVL-2.5-Instruct-72B~\cite{qwen2.5}  &
0.233/0.197 & 0.408/0.387 & 0.232/0.235 & 0.626/0.589 & 0.375/0.352 &
0.762/0.820 & -/- & 0.606/0.570 & 0.381/0.407 & 0.583/0.599 & 0.091/0.148 \\
QwenVL-3-Instruct-8B~\cite{qwen2.5}  &
0.156/0.094 & 0.280/0.170 & 0.191/0.121 & 0.507/0.388 & 0.283/0.193 &
0.761/0.822 & 0.612/0.604 & 0.723/0.696 & 0.434/0.427 & 0.633/0.637 & 0.033/0.044 \\
QwenVL-3-Instruct-32B~\cite{qwen2.5}  &
0.227/0.130 & 0.353/0.198 & 0.200/0.095 & 0.572/0.413 & 0.338/0.209 &
0.796/0.838 & 0.690/0.657 & 0.673/0.682 & 0.414/0.402 & 0.643/0.644 & 0.084/0.106 \\

\midrule
\multicolumn{1}{l}{\textit{\textbf{Specialized Models}}} &
\multicolumn{1}{c}{\textit{\textcolor{myred}{\textbf{In domain}}}} & \multicolumn{3}{c}{\textit{\textcolor{mygreen}{\textbf{Cross domain}}}} & \multicolumn{1}{c}{\textit{\textbf{Avg.}}} &
\multicolumn{1}{c}{\textit{\textcolor{myred}{\textbf{In domain}}}} & \multicolumn{3}{c}{\textit{\textcolor{mygreen}{\textbf{Cross domain}}}} & \multicolumn{1}{c}{\textit{\textbf{Avg.}}} &
\multicolumn{1}{c}{\textit{\textcolor{myred}{\textbf{In domain}}}} \\
ArtiMuse~\cite{artimuse}  &
\bluecellnp{70}0.614/0.627 & 0.397/0.385 & 0.230/0.232 & 0.349/0.334 & 0.398/0.395 &
-/- & -/- & -/- & -/- & -/- & -/- \\
DeQA~\cite{deqa_score}  &
-/- & -/- & -/- & -/- & -/- &
\bluecellnp{100}0.953/0.941 & 0.895/0.896 & 0.694/0.687 & 0.472/0.478 & 0.753/0.750 & -/- \\
Q-Align*~\cite{qalign}   &
0.551/0.573 & 0.398/0.386 & 0.194/0.197 & 0.137/0.123 & 0.320/0.320 &
0.941/0.940 & 0.886/0.887 & 0.674/0.684 & 0.403/0.419 & 0.726/0.733 & -/- \\
Q-Insight~\cite{Q-insight}  &
-/- & -/- & -/- & -/- & -/- &
0.933/0.916 & \bluecellnp{100}0.907/0.905 & \bluecellnp{70}0.742/0.736 & \bluecellnp{70}0.486/0.474 & \bluecellnp{70}0.767/0.758 & -/- \\
Q-Insight*~\cite{Q-insight}  &
0.228/0.175 & 0.405/0.376 & 0.212/0.217 & 0.617/0.537 & 0.366/0.326 &
0.733/0.750 & 0.800/0.938 & 0.580/0.548 & 0.369/0.368 & 0.621/0.651 & 0.060/0.152 \\
\midrule
\textbf{UniPercept (Ours)}   &
\textbf{\bluecellnp{100}{0.746/0.738}} & \textbf{\bluecellnp{100}0.589/0.577} & \textbf{\bluecellnp{100}0.336/0.346} & \textbf{\bluecellnp{100}0.688/0.681} & \textbf{\bluecellnp{100}0.590/0.586} &
\textbf{\bluecellnp{70}0.940/0.949} & \textbf{\bluecellnp{70}0.904/0.895} & \textbf{\bluecellnp{100}0.872/0.870} & \textbf{\bluecellnp{100}0.581/0.594} & \textbf{\bluecellnp{100}0.824/0.827} & \textbf{\bluecellnp{100}0.778/0.767} \\
\bottomrule[1.5pt]
\end{tabular}
\end{threeparttable}}
\label{tab:vr_leaderboard}
% \vspace{-15pt}
\end{table*}


To achieve precise alignment of the model across both Visual Rating (VR) and Visual Question Answering (VQA), we employ the GRPO algorithm~\cite{grpo} to perform \textbf{Task-Aligned RL} with task-specific reward functions for VR and VQA. For the VQA task, we adopt a binary reward:
% \vspace{-5pt}
\begin{equation}
r_{vqa} =
\begin{cases}
1, & \text{if the predicted answer is correct,} \\
0, & \text{otherwise.}
\end{cases}
\label{eq:vqa_reward}
\end{equation}
% \vspace{-5pt}

For the VR task, we design an \textbf{Adaptive Gaussian Soft Reward}, which continuously evaluates the prediction according to its numerical deviation from the ground truth:
% \vspace{-5pt}
\begin{equation}
r_{vr} = \exp\!\left(-\frac{(|p_i - g_i|)^2}{2\sigma_{\text{dyn}}^2}\right), \quad 
\sigma_{\text{dyn}} = \sigma_0 \left(1 + \alpha \frac{|p_i - g_i|}{100}\right),
\label{eq:vr_reward}
\end{equation}
% \vspace{-10pt}
where $p_i$ and $g_i$ denote the predicted and ground-truth scores (mapped to $[0,100]$), $\sigma_0$ is the base smoothing coefficient, and $\alpha$ controls the degree of adaptive Gaussian smoothing. This soft reward offers smoother gradients and avoids threshold-induced discontinuities. Following prior works~\cite{qalign,artimuse}, we adopt a \textit{Token As Score} strategy for VR, deriving ratings from the predicted token distribution.
We then incorporate this task-specific reward into the GRPO objective to enable perceptual-level policy optimization:

\begin{equation}
\begin{aligned}
\mathcal{J}^{\mathcal{B}}_{\text{GRPO}}(\theta)
&= \mathbb{E}_{\mathcal{B}}\!\Bigg[
\frac{1}{\sum_{i=1}^{G} |o^i|}
\sum_{i=1}^{G} \sum_{t=1}^{|o^i|}
r_i \cdot
\min\!\Big(
r_t^i(\theta)\hat{A}_t^i, \\
&\qquad\quad
\mathrm{clip}\big(r_t^i(\theta), 1-\epsilon, 1+\epsilon\big)\hat{A}_t^i
\Big)
\Bigg].
\end{aligned}
\label{eq:grpo_objective}
\end{equation}
% \vspace{-5pt}
where $r_t^i(\theta) = \frac{\pi_\theta(o_t^i|q^i,o_{<t}^i)}{\pi_{\text{old}}(o_t^i|q^i,o_{<t}^i)}$ is the ratio between current and old policies, $\hat{A}_t^i$ is the estimated advantage, and $r_i$ is the task-specific reward from Eq.~\ref{eq:vqa_reward} or Eq.~\ref{eq:vr_reward}. 
This unified formulation enables GRPO to align model behavior with both discrete correctness (VQA) and continuous perceptual consistency (VR).



% \vspace{-5pt}
\section{Experiments}
\label{sec:experiments}

\subsection{Implementation}
\label{sec:implementation}

\noindent\textbf{Evaluated Models.}
We evaluate a total of 18 models, encompassing three categories. (1) Proprietary Models: GPT-4o~\cite{gpt4}, Llama-4-Scout~\cite{meta_llama4_scout_2025}, Gemini-2.5-Pro~\cite{gemini}, Claude-Sonnet-4.5~\cite{claude} and Claude-Sonnet-4.5-Think~\cite{claude}. (2) Leading Open-Source Models: the InternVL3 and InternVL3.5 series~\cite{internvl3, internvl3-5}, QwenVL-2.5-Instruct and QwenVL-3-Instruct series~\cite{qwen2.5}, GLM-4.5-V-106BA12B~\cite{glm}, as well as LLaVA-OneVision-1.5-Instruct~\cite{LLaVA-OneVision-1.5}. (3) Specialized Models for IAA and IQA: Q-Align~\cite{qalign}, ArtiMuse~\cite{artimuse}, DeQA~\cite{deqa_score}, and Q-Insight~\cite{Q-insight}.


\noindent\textbf{Evaluation Settings.}
For VQA, all models were provided with identical prompts corresponding to each question, and their generated answers were compared against the ground-truth options.
For VR, we designed task-specific prompts for models lacking a dedicated scoring interface to elicit quantitative predictions, while specialized models for visual rating were directly evaluated through their native interfaces. It is worth noting that all specialized models are trained exclusively on \textit{In-domain} datasets.
For representative models (Q-Align and Q-Insight), we further retrain them on a mixed dataset comprising ArtiMuse-10K~\cite{artimuse}, KonIQ-10K~\cite{koniq}, and ISTA-10K to ensure consistent perceptual alignment across domains.


\noindent\textbf{Training Details.}
Based on InternVL3-8B\cite{internvl3}, UniPercept is trained in two stages as described in Sec.~\ref{sec:baseline}. 
The Domain-Adaptive Pre-Training stage adopts multiple public datasets, including APDDv2~\cite{apddv2} and Impressions~\cite{impressions} for IAA, Q-Ground-100K~\cite{q-ground} and DataDepictQA~\cite{depictqa_v2} for IQA, and DTD~\cite{dtd}, FMD~\cite{fmd}, Flickr2K~\cite{flickr2k}, and LSDIR~\cite{lsdir} for ISTA, among others. After preprocessing and filtering, the resulting corpus contains approximately 800K samples in total.
For Task-Aligned RL, we adopt the VR datasets ArtiMuse-10K~\cite{artimuse}, KonIQ-10K~\cite{koniq}, and ISTA-10K, along with $\sim$30K VQA samples generated as described in Sec.~\ref{sec:benchmark_construction}. 
Training is performed on 16 NVIDIA A100 GPUs for 2 epochs per each stage with a batch size of 128. 
In GRPO, we sample $n{=}8$ responses per query and set $\beta{=}0.001$, $\varepsilon{=}0.2$, and $\sigma{=}0.8$.


% \vspace{-5pt}
\subsection{Benchmark Results with Analysis}
\label{sec:benchmark_results}

\subsubsection{Visual Rating}
\label{sec:benchmark_results_vr}

\begin{table*}[t]
\centering
\small
% \caption{\textbf{Performance comparison of different models on UniPercept-Bench-VQA (IAA). }}
\caption{\textbf{Performance comparison of different models on UniPercept-Bench-VQA (IAA).} 
Category names are abbreviated; full definitions are provided in the Appendix. Results follow the same notation throughout the paper.}
\vspace{-6pt}
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\renewcommand{\arraystretch}{0.85} % 调整行距，默认1.0，数值越小行距越紧凑
\begin{tabular}{l|cccccccc|cccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{8}{c|}{\textbf{IAA Categories}} &
\multicolumn{6}{c|}{\textbf{QA Templates}} & \multirow{2}{*}{\textbf{Overall}} \\
\cmidrule(lr){2-9} \cmidrule(lr){10-15} 
 % & Comp. & VisStr. & Tech. & Creat. & Theme. & Emo. & Gest. & CompEv. &
 % Lv.Pred & How & What & Which & Why & Yes-No \\
 & \textit{Comp.} & \textit{VisStr.} & \textit{Tech.} & \textit{Creat.} & \textit{Theme.} & \textit{Emo.} & \textit{Gest.} & \textit{CompEv.} &
\textit{Lv.Pred} & \textit{How} & \textit{What} & \textit{Which} & \textit{Why} & \textit{Yes-No} \\
\midrule
\textit{Random Guess}  &  23.08\%  &  27.27\%  &  21.95\%  &  29.63\%  &  25.93\%  &  22.86\%  &  23.68\%  &  32.56\%  &  24.14\%  &  21.28\%  &  30.43\%  &  25.32\%  &  24.00\%  &  29.49\%  &  25.17\% \\
\multicolumn{16}{l}{\textit{\textbf{Proprietary Models}}} \\
GPT-4o  &  64.62\%  &  59.57\%  &  57.58\%  &  60.19\%  &  65.19\%  &  67.62\%  &  51.95\%  &  30.23\%  &  38.86\%  &  78.17\%  &  72.46\%  &  62.66\%  &  72.67\%  &  70.51\%  &  60.04\% \\
Llama-4-Scout &  62.56\%  &  68.45\%  &  59.76\%  &  61.11\%  &  57.78\%  &  70.48\%  &  48.68\%  &  32.56\%  &  43.97\%  &  70.92\%  &  69.57\%  &  61.39\%  &  77.33\%  &  70.51\%  &  60.91\% \\
Gemini-2.5-pro  & \bluecell{70}{71.79} &  68.45\%  &  61.59\%  & \bluecell{70}{76.85} &  67.41\%  &  63.81\%  & \bluecell{70}{61.84} &  37.21\%  &  45.98\%  &  78.72\%  &  73.91\%  &  67.72\%  &  84.67\%  &  \bluecell{100}{84.62} &  66.44\% \\
Claude-Sonnet-4.5  &  70.26\%  &  70.05\%  &  62.20\%  &  71.30\%  &  64.44\%  &  67.62\%  &  50.00\%  & \bluecell{70}{46.51} & \bluecell{70}{46.84} &  77.30\%  &  76.09\%  &  65.19\%  &  86.00\%  &  69.23\%  &  65.45\% \\
Claude-Sonnet-4.5-Think  &  71.28\%  &  69.52\%  &  61.21\%  &  68.52\%  &  62.22\%  &  66.67\%  &  53.25\%  &  41.86\%  &  44.57\%  &  75.89\%  &  77.54\%  &  67.09\%  &  86.00\%  &  66.67\%  &  64.73\% \\
\midrule
\multicolumn{16}{l}{\textit{\textbf{Open-Source Models}}} \\
LLaVA-OneVision-1.5-Instruct-8B  &  67.18\%  &  68.62\%  &  61.21\%  &  62.96\%  &  67.41\%  &  62.86\%  &  53.25\%  &  20.93\%  &  34.86\%  &  85.21\%  &  79.71\%  &  65.82\%  &  83.33\%  &  69.23\%  &  62.60\% \\
GLM-4.5-V-106BA12B  &  67.18\%  &  65.78\%  &  60.98\%  &  75.00\%  &  64.44\%  &  68.57\%  &  51.32\%  &  \bluecell{70}{46.51} &  45.40\%  &  71.63\%  &  78.26\%  &  65.82\%  &  84.67\%  &  70.51\%  &  64.46\% \\
InternVL3-8B  &  65.64\%  &  67.55\%  &  59.39\%  &  67.59\%  &  69.63\%  &  62.86\%  &  50.65\%  &  25.58\%  &  36.00\%  &  81.69\%  &  73.91\%  &  67.72\%  &  86.00\%  &  71.79\%  &  62.60\% \\
InternVL3-78B  & \bluecell{70}{71.79} & \bluecell{70}{73.26} &  61.21\%  &  73.15\%  & \bluecell{70}{74.81} & \bluecell{70}{74.29} &  53.25\%  &  37.21\%  &  45.14\%  &  85.82\%  & \bluecell{70}{81.16} &  72.15\%  &  86.00\%  &  75.64\%  & \bluecell{70}{68.28} \\
InternVL3.5-8B  &  32.31\%  &  29.41\%  &  30.30\%  &  26.85\%  &  28.89\%  &  26.67\%  &  23.38\%  &  9.30\%  &  17.14\%  &  41.13\%  &  26.81\%  &  19.62\%  &  36.00\%  &  58.97\%  &  28.18\% \\
InternVL3.5-38B  &  37.44\%  &  40.11\%  &  27.88\%  &  39.81\%  &  34.81\%  &  38.10\%  &  45.45\%  &  6.98\%  &  34.00\%  &  47.52\%  &  26.09\%  &  28.48\%  &  37.33\%  &  50.00\%  &  35.67\% \\
QwenVL-2.5-Instruct-7B  &  67.18\%  &  70.74\%  &  56.36\%  &  66.67\%  &  68.89\%  &  63.81\%  &  48.05\%  &  37.21\%  &  38.86\%  &  76.76\%  &  75.36\%  &  67.09\%  &  \bluecell{100}{87.33} &  71.79\%  &  63.19\% \\
QwenVL-2.5-Instruct-72B  &  22.05\%  &  24.60\%  &  25.45\%  &  29.63\%  &  30.37\%  &  18.10\%  &  19.48\%  &  6.98\%  &  14.00\%  &  19.86\%  &  17.39\%  &  24.05\%  &  41.33\%  &  51.28\%  &  23.74\% \\
QwenVL-3-Instruct-8B  &  31.28\%  &  32.09\%  &  32.12\%  &  37.04\%  &  34.07\%  &  22.86\%  &  37.66\%  &  25.58\%  &  35.43\%  &  14.89\%  &  17.39\%  &  34.81\%  &  28.67\%  &  73.08\%  &  31.92\% \\
QwenVL-3-Instruct-32B  &  23.08\%  &  26.74\%  &  32.12\%  &  26.85\%  &  32.59\%  &  20.95\%  &  33.77\%  &  20.93\%  &  33.43\%  &  9.22\%  &  13.77\%  &  31.01\%  &  18.67\%  &  66.67\%  &  27.39\% \\
\midrule
\multicolumn{16}{l}{\textit{\textbf{Specialized Models}}} \\
ArtiMuse  &  67.69\%  &  68.45\%  &  \bluecell{70}{64.85}  &  74.07\%  &  71.85\%  &  64.76\%  &  61.04\%  &  32.56\%  &  39.14\%  & \bluecell{70}{88.65} &  76.81\%  & \bluecell{70}{72.78} &  85.33\%  &  \bluecell{70}{79.49}  &  66.31\% \\
\midrule
\textbf{UniPercept (Ours)}  & \textbf{\bluecell{100}{80.00}} & \textbf{\bluecell{100}{77.54}} & \textbf{\bluecell{100}{69.70}} & \textbf{\bluecell{100}{80.56}} & \textbf{\bluecell{100}{79.26}} & \textbf{\bluecell{100}{80.95}} & \textbf{\bluecell{100}{67.53}} & \textbf{\bluecell{100}{69.77}} & \textbf{\bluecell{100}{63.71}} & \textbf{\bluecell{100}{92.20}} & \textbf{\bluecell{100}{81.88}} & \textbf{\bluecell{100}{75.32}} & \textbf{\bluecell{70}{86.67}} & \textbf{\bluecell{100}{84.62}} & \textbf{\bluecell{100}{76.55}} \\
\bottomrule[1.5pt]
\end{tabular}
\end{threeparttable}}
\label{tab:vqa_iaa_leaderboard}
% \vspace{-10pt}
\end{table*}


\begin{figure*}[htbp]
\centering
\begin{minipage}[t]{0.72\textwidth}  % 表格区域稍宽
    \vspace{0pt}  % 保证顶部对齐
    \centering
    \small
    \captionof{table}{\textbf{Performance comparison of different models on UniPercept-Bench-VQA (IQA).}}
    \vspace{-6pt}
    \resizebox{\textwidth}{!}{%
    % === 你的表格内容 ===
    \begin{threeparttable}
\renewcommand{\arraystretch}{0.9} % 调整行距
\begin{tabular}{l|ccc|cccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{3}{c|}{\textbf{IQA Categories}} &
\multicolumn{6}{c|}{\textbf{QA Templates}} &
\multirow{2}{*}{\textbf{Overall}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-10}
 % & Loc. & Sev. & Type. & Lv.Pred & How & What & Which & Why & Yes-No \\
 & \textit{Loc.} & \textit{Sev.} & \textit{Type.} & \textit{Lv.Pred} & \textit{How} & \textit{What} & \textit{Which} & \textit{Why} & \textit{Yes-No} \\
\midrule
\textit{Random Guess}   &
23.67\%  &  24.75\%  &  20.08\%  &  24.75\%  &
27.03\%  &  16.05\%  &  25.00\%  &  21.39\%  &
22.99\%  &  23.16\% \\
\multicolumn{11}{l}{\textit{\textbf{Proprietary Models}}} \\
GPT-4o   &
71.74\%  &  53.18\%  &  70.49\%  &  53.18\%  &
83.78\%  &  59.26\%  &  61.31\%  &  80.21\%  &
67.82\%  &  66.36\% \\
Llama-4-Scout   &
60.18\%  &  58.19\%  &  52.05\%  &  58.19\%  &
82.16\%  &  37.04\%  &  38.69\%  &  66.31\%  &
62.07\%  &  57.81\% \\
Gemini-2.5-pro   &
32.84\%  &  52.84\%  &  40.98\%  &  52.84\%  &
40.54\%  &  32.72\%  &  29.17\%  &  41.18\%  &
28.74\%  &  40.17\% \\
Claude-Sonnet-4.5   &
71.19\%  &  51.51\%  &  66.80\%  &  51.51\%  &
90.81\%  &  50.00\%  &  50.60\%  &  82.89\%  &
71.26\%  &  64.80\% \\
Claude-Sonnet-4.5-Think   &
71.19\%  &  55.52\%  &  66.80\%  &  55.52\%  &
89.19\%  &  50.00\%  &  51.79\%  &  82.89\%  &
72.41\%  &  65.90\% \\
\midrule
\multicolumn{11}{l}{\textit{\textbf{Open-Source Models}}} \\
LLaVA-OneVision-1.5-Instruct-8B   &
\bluecell{70}{76.51}  &  \bluecell{70}{59.87}  &  77.46\%  &  \bluecell{70}{59.87}  &
\bluecell{70}{91.35}  &  \bluecell{70}{70.37}  &  61.31\%  &  82.35\%  &
75.86\%  &  \bluecell{70}{72.15} \\
GLM-4.5-V-106BA12B   &
70.09\%  &  35.79\%  &  54.51\%  &  35.79\%  &
88.11\%  &  48.77\%  &  44.05\%  &  74.33\%  &
68.97\%  &  57.17\% \\
InternVL3-8B   &
71.56\%  &  52.84\%  &  59.43\%  &  52.84\%  &
87.03\%  &  59.88\%  &  48.81\%  &  71.12\%  &
71.26\%  &  63.69\% \\
InternVL3-78B   &
75.41\%  &  51.84\%  &  \bluecell{70}{81.56}  &  51.84\%  &
\bluecell{100}{93.51}  &  66.67\%  &  \bluecell{70}{63.10}  &  \bluecell{100}{88.24}  &
66.67\%  &  70.31\% \\
InternVL3.5-8B   &
38.17\%  &  44.82\%  &  38.11\%  &  44.82\%  &
35.14\%  &  41.98\%  &  30.36\%  &  36.36\%  &
56.32\%  &  39.98\% \\
InternVL3.5-38B   &
38.90\%  &  49.83\%  &  45.08\%  &  49.83\%  &
46.49\%  &  41.36\%  &  31.55\%  &  33.16\%  &
62.07\%  &  43.29\% \\
QwenVL-2.5-Instruct-7B   &
74.13\%  &  48.83\%  &  66.39\%  &  48.83\%  &
88.65\%  &  60.49\%  &  53.57\%  &  78.61\%  &
\bluecell{70}{77.01}  &  65.44\% \\
QwenVL-2.5-Instruct-72B   &
31.01\%  &  4.68\%  &  16.39\%  &  4.68\%  &
35.14\%  &  14.81\%  &  11.31\%  &  22.99\%  &
66.67\%  &  20.50\% \\
QwenVL-3-Instruct-8B   &
34.68\%  &  55.18\%  &  16.39\%  &  55.18\%  &
20.54\%  &  18.52\%  &  27.38\%  &  25.67\%  &
\bluecell{70}{77.01}  &  36.21\% \\
QwenVL-3-Instruct-32B   &
29.54\%  &  14.38\%  &  16.80\%  &  14.38\%  &
11.89\%  &  18.52\%  &  25.60\%  &  22.46\%  &
74.71\%  &  22.52\% \\
\midrule
\textbf{UniPercept (Ours)}   &
\textbf{\bluecell{100}{77.43}}  &  \textbf{\bluecell{100}{79.60}}  &  \textbf{\bluecell{100}{90.98}}  &  \textbf{\bluecell{100}{79.60}}  &
\textbf{87.03\%}  &  \textbf{\bluecell{100}{80.86}}  &  \textbf{\bluecell{100}{75.60}}  &  \textbf{\bluecell{70}{83.42}}  &
\textbf{\bluecell{100}{79.31}}  &  \textbf{\bluecell{100}{81.07}} \\
\bottomrule[1.5pt]
\end{tabular}
\end{threeparttable}}
\label{tab:vqa_iqa_leaderboard}
\end{minipage}
\hfill
\begin{minipage}[t]{0.27\textwidth}  % 图像区域稍窄
    \vspace{0pt}  % 顶部对齐
    \centering
    \includegraphics[width=\linewidth]{unipercept/Figures/exp/circular_bar_unipercept_v2.pdf}
    \vspace{-20pt}
    \caption{\textbf{Results on UniPercept-Bench.} 
    VQA and VR are evaluated by Acc. and $(SRCC+PLCC)/2$.}
    \label{fig:benchmark_results_radar}
\end{minipage}
% \vspace{-10pt}
\end{figure*}


\begin{table*}[htbp]
\centering
\scriptsize  % 比 small 更小
\caption{\textbf{Performance comparison of different models on UniPercept-Bench-VQA (ISTA).}}
\vspace{-6pt}
\label{tab:vqa_ista_leaderboard}

\begin{threeparttable}
\renewcommand{\arraystretch}{0.75}   % 行距再压一点
\setlength{\tabcolsep}{2pt}         % 列间距再收紧一点

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l|ccccc|ccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{5}{c|}{\textbf{ISTA Categories}} &
\multicolumn{5}{c|}{\textbf{QA Templates}} &
\multirow{2}{*}{\textbf{Overall}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
 & \textit{Scene.} & \textit{Phys.} & \textit{Mat.} & \textit{Geo.} & \textit{Sem.} &
   \textit{How} & \textit{What} & \textit{Which} & \textit{Why} & \textit{Yes-No} \\
\midrule
\textit{Random Guess}   & 26.50\% & 23.63\% & 24.73\% & 30.30\% & 30.58\% & 26.28\% & 23.84\% & 24.29\% & 33.77\% & 33.33\% & 26.60\% \\
\multicolumn{12}{l}{\textit{\textbf{Proprietary Models}}} \\
GPT-4o                 & 75.64\% & 79.12\% & 73.48\% & 33.33\% & 77.27\% & 71.79\% & 78.78\% & 69.23\% & 77.92\% & 72.46\% & 74.64\% \\
Llama-4-Scout          & 73.50\% & 75.27\% & 71.68\% & 72.73\% & 67.77\% & 75.64\% & 69.77\% & 69.64\% & 77.27\% & 69.57\% & 71.86\% \\
Gemini-2.5-pro         & 76.50\% & 82.42\% & 77.06\% & 66.67\% & 77.69\% & 78.21\% & 78.20\% & 75.71\% & 82.47\% & 71.01\% & 77.73\% \\
Claude-Sonnet-4.5      & 76.92\% & 78.57\% & 74.91\% & \bluecell{70}{90.91} & 77.69\% &
                         76.92\% & 77.03\% & 74.49\% & 81.82\% & 79.71\% & 77.32\% \\
Claude-Sonnet-4.5-Think& 77.35\% & 78.02\% & 73.12\% & 87.88\% & 75.21\% &
                         76.28\% & 74.71\% & 74.09\% & 81.82\% & 76.81\% & 76.08\% \\
\midrule
\multicolumn{12}{l}{\textit{\textbf{Open-Source Models}}} \\
LLaVA-OneVision-1.5-Instruct-8B & 78.63\% & \bluecell{70}{85.16} & \bluecell{100}{82.44} & 72.73\% & \bluecell{100}{80.17} &
                                   \bluecell{100}{83.33} & \bluecell{70}{81.40} & 75.30\% & \bluecell{100}{84.42} & \bluecell{100}{88.41} & \bluecell{70}{81.13} \\
GLM-4.5-V-106BA12B              & \bluecell{70}{81.20} & 79.67\% & 74.55\% & 72.73\% & 75.21\% &
                                   80.77\% & 76.74\% & 73.68\% & 79.87\% & 78.26\% & 77.22\% \\
InternVL3-8B                    & 75.64\% & 79.12\% & 73.48\% & 33.33\% & 77.27\% &
                                   71.79\% & 78.78\% & 69.23\% & 77.92\% & 72.46\% & 74.64\% \\
InternVL3-78B                   & 79.06\% & \bluecell{70}{85.16} & \bluecell{70}{77.42} & 69.70\% & \bluecell{70}{78.51} &
                                   81.41\% & 79.65\% & 73.68\% & \bluecell{100}{84.42} & 81.16\% & 79.28\% \\
InternVL3.5-8B                  & 54.27\% & 50.55\% & 58.42\% & 39.39\% & 36.36\% &
                                   46.79\% & 56.69\% & 48.58\% & 29.87\% & 71.01\% & 49.79\% \\
InternVL3.5-38B                 & 50.00\% & 55.49\% & 61.29\% & 30.30\% & 35.95\% &
                                   50.64\% & 59.30\% & 42.91\% & 37.01\% & 57.97\% & 50.10\% \\
QwenVL-2.5-Instruct-7B          & 74.79\% & 72.53\% & 74.91\% & 51.52\% & 73.55\% &
                                   73.72\% & 77.33\% & 66.80\% & 74.03\% & 73.91\% & 73.30\% \\
QwenVL-2.5-Instruct-72B         & 14.10\% & 29.12\% & 19.71\% & 12.12\% & 18.60\% &
                                   20.51\% & 12.21\% & 14.57\% & 31.17\% & 46.38\% & 19.59\% \\
QwenVL-3-Instruct-8B            & 27.78\% & 32.42\% & 25.45\% & 39.39\% & 24.79\% &
                                   14.74\% & 23.26\% & 28.34\% & 25.32\% & 81.16\% & 27.63\% \\
QwenVL-3-Instruct-32B           & 26.50\% & 24.73\% & 19.00\% & 15.15\% & 18.60\% &
                                   11.54\% & 18.31\% & 22.67\% & 17.53\% & 66.67\% & 21.65\% \\
\midrule
\rowcolor{tableblue!8}  % 整行浅蓝底，避免蓝色 cell 中间出现白条
\textbf{UniPercept (Ours)} &
  \textbf{\bluecell{100}{89.74}} &
  \textbf{\bluecell{100}{85.71}} &
  \textbf{\bluecell{100}{82.44}} &
  \textbf{\bluecell{100}{93.94}} &
  \textbf{\bluecell{70}{78.51}}  &
  \textbf{\bluecell{70}{82.69}}  &
  \textbf{\bluecell{100}{89.24}} &
  \textbf{\bluecell{100}{78.54}} &
  \textbf{\bluecell{70}{83.12}}  &
  \textbf{\bluecell{70}{85.51}}  &
  \textbf{\bluecell{100}{84.23}} \\
\bottomrule[1.5pt]
\end{tabular*}
\end{threeparttable}

% \vspace{-15pt}
\end{table*}

\noindent\textbf{General Models vs. Specialized Models.}
Visual Rating is a challenging task that requires models to output continuous, high-precision perceptual scores. 
As shown in Table~\ref{tab:vr_leaderboard}, most \textit{general-purpose MLLMs} without task-specific training exhibit significantly lower performance compared with \textit{specialized models}. 
This gap arises from the inherent difficulty of directly generating numerical outputs in text form, which often leads to hallucinated or unstable predictions---a phenomenon also discussed in prior works~\cite{qalign,nexttoken,artimuse}. 
In contrast, specialized methods adopt structured strategies such as \textit{Token As Score}, effectively stabilizing the regression behavior of large models on continuous scales.~\cite{qalign,artimuse}

\noindent\textbf{Domain-wise Analysis.}
Model performance varies significantly across different domains, reflecting differences in task objectivity. 
IQA achieves the highest correlations, followed by ISTA, while IAA remains the most challenging due to its subjective and ambiguous aesthetic judgments. 
These results suggest that perceptual-level visual rating becomes increasingly difficult as the task shifts from objective assessment toward subjective reasoning.


% \vspace{-5pt}
\subsubsection{Visual Question Answering}
\label{sec:benchmark_results_vqa}
% \vspace{-5pt}

\noindent\textbf{Domain-wise Analysis.}
Across domains, the best-performing generalized models can reach accuracies of up to 68.28\%, 72.15\%, and 81.13\% on IAA, IQA, and ISTA, respectively. 
However, their average accuracies drop to only \textbf{51.62\%}, \textbf{51.45\%}, and \textbf{60.56\%}. 
This disparity suggests that perceptual-level visual question answering remains highly challenging for current MLLMs, as they often rely on unstable domain-specific heuristics rather than robust perceptual reasoning. 
Among the three domains, ISTA appears slightly easier, as it centers on objective and physically grounded properties—such as geometry, structure, and material composition—that align better with the visual–text priors learned during large-scale pretraining. In contrast, IAA and IQA require subjective reasoning over aesthetics, emotion, and perceptual quality—nuanced judgments that general models are not explicitly optimized for.


\noindent\textbf{Category-wise Analysis.}
Models generally perform better on holistic perception categories such as \textit{Composition \& Design} and \textit{Theme \& Communication}, which focus on the overall aesthetic and semantic coherence of an image. 
Most models achieve accuracies above \textbf{60\%} in these categories, indicating that global scene perception is relatively well captured by vision–language pretraining. 
In contrast, performance drops substantially on fine-grained perceptual categories such as \textit{Overall Gestalt}, \textit{Material Representation}, and \textit{Geometric Composition}, where most models remain below \textbf{50\%}. 
These results suggest that while high-level holistic understanding is well learned, precise reasoning over local structures cues remains a key limitation. 


\noindent\textbf{QA Template Analysis.}
The \textit{Level Prediction} questions require models to provide fine-grained evaluations of images along specific dimensions (as shown in Fig.~\ref{fig:qa_example}). 
Due to the demand for precise quantitative reasoning, most MLLMs struggle with this type, achieving only around \textbf{36\%} and \textbf{45\%} average accuracy on the IAA and IQA domains, respectively. 
For other QA templates, “\textit{Yes-No}” and “\textit{Why}” questions—closer to higher-level reasoning and causal inference—allow generalized MLLMs to reach average accuracies above \textbf{60\%}. 
In contrast, “\textit{What}” and “\textit{Which}” questions, which require detailed and localized visual analysis, remain challenging, reflecting the current models’ limited capacity for fine-grained perceptual understanding.

% \vspace{-5}
\subsection{Further Discussion on UniPercept}
% \vspace{-5pt}
\subsubsection{Performance}
\label{sec:performance_unipercept}

As shown in Fig.~\ref{fig:benchmark_results_radar} and Tabs.~\ref{tab:vr_leaderboard},~\ref{tab:vqa_iaa_leaderboard}, ~\ref{tab:vqa_iqa_leaderboard}, and  ~\ref{tab:vqa_ista_leaderboard}, UniPercept is capable of handling both major types of perceptual-level image understanding tasks (\textit{VR} \& \textit{VQA}) across the three perceptual domains of \textit{IAA}, \textit{IQA}, and \textit{ISTA}. 
Benefiting from the proposed \textbf{Domain-Adaptive Pre-Training} and \textbf{Task-Aligned RL} strategies, UniPercept consistently outperforms both generalized and specialized models. 
It not only achieves strong in-domain results but also exhibits remarkable cross-domain generalization, demonstrating its capability as a unified perceptual understanding baseline.

\begin{table*}[t]
\vspace{-10pt}
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.9}
\caption{\textbf{More Performance Results of FLUX.1-dev w/ UniPercept Reward.}}
\label{tab:application}
\vspace{-6pt}

\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l cc c cc ccc}
\toprule
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{2}{c}{\textbf{Preference Score}} &
\multicolumn{1}{c}{\textbf{Image Quality}} &
\multicolumn{2}{c}{\textbf{Image Aesthetics}} &
\multicolumn{3}{c}{\textbf{UniPercept Score}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-4}
\cmidrule(lr){5-6} \cmidrule(lr){7-9}
& PickScore~\cite{pickscore} & HPSv3~\cite{hspv3} & DeQA~\cite{deqa_score} & LAION-Aes~\cite{laion-aes} & ArtiMuse~\cite{artimuse} & IAA & IQA & ISTA \\
\midrule
Baseline 
& 22.46 & 10.71 & 4.32 & 5.77  & 59.02 & 65.18 & 73.59 & 46.64 \\

w/ UniPercept IAA Reward 
& 22.47 & 10.09 & 4.09 & \bluecellnp{100}{6.19} & \bluecellnp{100}{67.02} & \bluecellnp{100}{76.20} & 76.39 & 54.83 \\

w/ UniPercept IQA Reward  
& 22.63 & \bluecellnp{100}{11.21} & \bluecellnp{100}{4.37} & 6.02 & 63.64 & 72.16 & \bluecellnp{70}{76.87} & 52.34 \\

w/ UniPercept ISTA Reward  
& \bluecellnp{100}{22.72} & \bluecellnp{70}{11.09} & \bluecellnp{100}{4.37} & \bluecellnp{70}{6.16} & 63.75 & 72.23 & 76.17 & \bluecellnp{100}{59.61} \\

\textbf{w/ UniPercept Reward (All)} 
& \textbf{\bluecellnp{70}{22.67}} 
& \textbf{10.93} 
& \textbf{\bluecellnp{70}{4.33}} 
& \textbf{\bluecellnp{100}{6.19}} 
& \textbf{\bluecellnp{70}{65.52}} 
& \textbf{\bluecellnp{70}{74.24}} 
& \textbf{\bluecellnp{100}{77.04}} 
& \textbf{\bluecellnp{70}{59.08}} \\
\bottomrule
\end{tabular}
}

% \vspace{-12pt}
\end{table*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{unipercept/Figures/appendix/application_appendix.pdf}
    \vspace{-6pt}
    \caption{\textbf{More results of FLUX.1-dev w/ UniPercept Reward.} Different reward signals emphasize distinct perceptual attributes, while \textit{UniPercept Reward (All)} achieves the best overall performance by integrating complementary perceptual cues.}
    \label{fig:application_appendix}
\end{figure*}

\subsubsection{UniPercept Reward}
\label{sec:result_reward}

We investigate the use of UniPercept as a \textbf{multi-dimensional perceptual reward model} for text-to-image generation. UniPercept provides three types of visual ratings (Aesthetics Quality (IAA), Image Quality (IQA), and Structure \& Texture Richness (ISTA)) which can be employed as independent reward signals or jointly as an integrated perceptual reward. All reward configurations are incorporated into the Flow-GRPO~\cite{liu2025flowgrpotrainingflowmatching} fine-tuning pipeline based on FLUX.1-dev~\cite{flux}. Quantitative results in Tab.~\ref{tab:application} show that each reward captures a distinct facet of perceptual evaluation and thus leads to different characteristic improvements. The IAA reward mainly enhances aesthetics-related metrics, whereas the IQA reward yields stronger gains on quality-oriented metrics such as sharpness and clarity. The ISTA reward, in contrast, provides more balanced improvements across all dimensions due to its emphasis on structural and textural richness. When combining all three as a unified UniPercept reward (All), the model integrates the benefits of each dimension and achieves the best overall performance.

Corresponding qualitative results in Fig.~\ref{fig:application_appendix} further demonstrate that UniPercept-guided training improves visual fidelity, perceptual quality, and human preference. These results confirm that UniPercept serves effectively not only as a reward model but also as a unified set of perceptual metrics for evaluating generated images.

\subsubsection{UniPercept Metrics}
\label{sec:metrics}

% 对于现有各类生成模型的分析，取若干模型在DPG GenEval上进行测试，给出三个维度的metric分数
\noindent\textbf{For Models.}
UniPercept can serve as an perceptual‐level metric that assesses the quality of outputs from any model producing images, covering three complementary dimensions: IAA, IQA, and ISTA. Here, we take text-to-image models as an example and apply UniPercept as an evaluation metric on both the DPG~\cite{dpg} and GenEval~\cite{geneval} benchmarks to measure the perceptual quality of generated images. Except for special cases (e.g., GPT-Image-1~\cite{gpt4}, where output resolution cannot be controlled), all models are evaluated with a fixed output resolution of 1024×1024. The results are reported in Tab.\ref{tab:dpg_unipercept_full} and Tab.\ref{tab:geneval_unipercept_full}.

We observe that while current models generally achieve strong performance in IQA, there remains \textbf{substantial room for improvement in IAA and ISTA}. Moreover, as model capability advances, we see consistent improvements in both instruction-following ability (as reflected by DPG and GenEval metrics) and perceptual image quality (as reflected by UniPercept). For instance, GPT-Image-1~\cite{gpt4} and Qwen-Image~\cite{wu2025qwenimagetechnicalreport} exhibit strong performance across both Dataset Metrics and UniPercept Metrics. More detailed analyses will be presented in future work.


\begin{table*}[t]
\centering
\small
\caption{\textbf{Evaluation of T2I Models on DPG~\cite{dpg} Metrics and UniPercept Metrics.}}
\vspace{-6pt}
\resizebox{0.95\textwidth}{!}{
\begin{threeparttable}[t]
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{l|cccccc|cccc}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{6}{c|}{\textbf{DPG Metrics~\cite{dpg}}} &
\multicolumn{4}{c}{\textbf{UniPercept Metrics}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-11}
 & \textbf{Global} & \textbf{Entity} & \textbf{Attribute} & \textbf{Relation} & \textbf{Other} & \textbf{Overall} 
 & \textbf{IAA} & \textbf{IQA} & \textbf{ISTA} & \textbf{Avg.} \\
\midrule

OmniGen~\cite{OmniGen}                
& -- & -- & -- & -- & -- & -- 
& 62.83 & 72.22 & 45.09 & 60.04 \\

OmniGen2~\cite{OmniGen2}               
& 88.81 & 88.83 & 90.18 & 89.37 & 90.27 & 83.57
& 58.51 & 71.89 & 43.31 & 57.90 \\

BAGEL~\cite{bagel}                  
& \bluecellnp{70}{88.94} & 90.37 & \bluecellnp{70}{91.29} & 90.82 & 88.67 & 85.07
& 60.20 & 70.52 & 45.78 & 58.83 \\

SANA-1.6B~\cite{xie2024sana,xie2025sana}              
& 86.00 & 91.50 & 88.90 & 91.90 & 90.70 & 84.80
& 40.33 & 42.89 & 42.41 & 41.87 \\

Lumina-DiMOO~\cite{dimoo}           
& 81.46 & \bluecellnp{100}{92.08} & 88.98 & \bluecellnp{100}{94.31} & 82.00 & \bluecellnp{70}{86.04}
& 61.00 & 71.14 & 44.83 & 58.99 \\

FLUX.1-dev~\cite{flux}             
& 74.35 & 90.00 & 88.96 & 90.87 & 88.33 & 83.84
& \bluecellnp{100}{65.18} & \bluecellnp{100}{73.59} & \bluecellnp{70}{46.64} & \bluecellnp{100}{61.80} \\

% FLUX.1-Kontext~\cite{flux}         
% & -- & -- & -- & -- & -- & --  
% & 59.88 & 72.46 & 44.76 & 59.03 \\

GPT-Image-1~\cite{gpt4}            
& 88.89 & 88.94 & 89.84 & \bluecellnp{70}{92.63} & \bluecellnp{70}{90.96} & 85.15
& 62.27 & \bluecellnp{100}{72.87} & 44.88 & 60.00 \\

Qwen-Image~\cite{wu2025qwenimagetechnicalreport}             
& \bluecellnp{100}{91.32} & \bluecellnp{70}{91.56} & \bluecellnp{100}{92.02} & \bluecellnp{100}{94.31} & \bluecellnp{100}{92.73} & \bluecellnp{100}{88.32}
& \bluecellnp{70}{62.89} & 72.15 & \bluecellnp{100}{47.23} & \bluecellnp{70}{60.76} \\

\bottomrule[1.5pt]
\end{tabular}

\end{threeparttable}}
\label{tab:dpg_unipercept_full}
\end{table*}

\begin{table*}[htbp]
\centering
\small
\caption{\textbf{Evaluation of T2I Models on GenEval~\cite{geneval} Metrics and UniPercept Metrics.}}
\vspace{-6pt}
\resizebox{0.95\textwidth}{!}{
\begin{threeparttable}[t]
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{l|ccccccc|cccc}
\toprule[1.5pt]
\multirow{2}{*}{\textbf{Models}} &
\multicolumn{7}{c|}{\textbf{GenEval~\cite{geneval} Metrics}} &
\multicolumn{4}{c}{\textbf{UniPercept Metrics}} \\
\cmidrule(lr){2-8} \cmidrule(lr){9-12}
& \textbf{Single Obj.} & \textbf{Two Obj.} & \textbf{Counting} & \textbf{Colors} & \textbf{Position} & \textbf{Attr. Bind.} & \textbf{Overall}
& \textbf{IAA} & \textbf{IQA} & \textbf{ISTA} & \textbf{Avg.} \\
\midrule

OmniGen~\cite{OmniGen}
& \bluecellnp{70}{0.99} & 0.86 & 0.64 & 0.85 & 0.31 & 0.55 & 0.70
& 58.84 & \bluecellnp{70}{75.62} & 41.00 & 58.49 \\

OmniGen2~\cite{OmniGen2}
& \bluecellnp{70}{0.99} & \bluecellnp{100}{0.96} & 0.74 & \bluecellnp{100}{0.98} & 0.71 & 0.75 & 0.86
& 54.20 & 75.16 & 34.48 & 54.61 \\

BAGEL~\cite{bagel}
& \bluecellnp{70}{0.99} & \bluecellnp{70}{0.94} & 0.81 & 0.88 & 0.64 & 0.63 & 0.82
& 58.68 & 71.24 & 38.35 & 56.09 \\

SANA-1.6B~\cite{xie2024sana,xie2025sana}
& \bluecellnp{70}{0.99} & 0.77 & 0.62 & 0.88 & 0.21 & 0.47 & 0.66
& 34.34 & 35.11 & 31.22 & 33.56 \\

Lumina-DiMOO~\cite{dimoo}
& \bluecellnp{100}{1.00} & \bluecellnp{70}{0.94} & \bluecellnp{70}{0.85} & 0.89 & \bluecellnp{100}{0.85} & \bluecellnp{70}{0.76} & \bluecellnp{100}{0.88}
& 51.93 & 71.98 & 30.86 & 51.59 \\

FLUX.1-dev~\cite{flux}
& 0.98 & 0.81 & 0.74 & 0.79 & 0.22 & 0.45 & 0.66
& \bluecellnp{70}{64.24} & 74.96 & \bluecellnp{70}{41.14} & \bluecellnp{70}{60.11} \\

% FLUX.1-Kontext~\cite{flux}
% & -- & -- & -- & -- & -- & -- & --
% & 54.41 & 75.19 & 33.87 & 54.49 \\

GPT-Image-1~\cite{gpt4}
& \bluecellnp{70}{0.99} & 0.92 & \bluecellnp{70}{0.85} & \bluecellnp{70}{0.92} & 0.75 & 0.61 & 0.84
& \bluecellnp{100}{69.07} & \bluecellnp{100}{76.74} & \bluecellnp{100}{51.26} & \bluecellnp{100}{65.69} \\

Qwen-Image~\cite{wu2025qwenimagetechnicalreport}
& \bluecellnp{70}{0.99} & 0.92 & \bluecellnp{100}{0.89} & 0.88 & \bluecellnp{70}{0.76} & \bluecellnp{100}{0.77} & \bluecellnp{70}{0.87}
& 52.02 & 74.44 & 34.13 & 53.53 \\

\bottomrule[1.5pt]
\end{tabular}

\end{threeparttable}}
\label{tab:geneval_unipercept_full}
\end{table*}



% 对于现有各类数据集的分析，测试下现有数据集的unipecept metrics的分布
\noindent\textbf{For Datasets.}
We evaluate a variety of natural-image and AIGC-image datasets using UniPercept as the assessment metric, with results summarized in Tab.\ref{tab:metrics_dataset}. Among all datasets, Unsplash~\cite{unsplash} and Blip3o-60K\cite{chen2025blip3ofamilyfullyopen} achieve the strongest overall performance across the three domains of IAA, IQA, and ISTA. A more in-depth investigation of these distributional characteristics is left for future work.
% 我们对于常见的自然图像数据集和AIGC图像数据集使用UniPercept 作为Metrics进行了评估，结果展示在Tab.~\ref{tab:metrics_dataset}. 可以看到自然图像和真实图像的分布有所不同，同时评估结果显示Unsplash和Blip3o-60K~\cite{chen2025blip3ofamilyfullyopen}在IAA，IQA，ISTA三个方面的综合表现领先于其他dataset。进一步的探究留在future work中。

\begin{table}[htbp]
\centering
\small
\caption{\textbf{UniPercept Metrics on Various Datasets.}}
\vspace{-6pt}
\label{tab:metrics_dataset}
\resizebox{0.49\textwidth}{!}{
\begin{threeparttable}[t]
\renewcommand{\arraystretch}{0.9}

\begin{tabular}{l|cccc}
\toprule[1.5pt]
\textbf{Dataset} & \textbf{UniPercept-IAA} & \textbf{UniPercept-IQA} & \textbf{UniPercept-ISTA} & \textbf{Avg.} \\
\midrule

\multicolumn{5}{l}{\textit{\textbf{Natural Images}}} \\
ImageNet~\cite{russakovsky2015imagenetlargescalevisual}   
& 53.88 & 61.90 & 36.79 & 50.85 \\

Unsplash~\cite{unsplash}   
& \bluecellnp{70}{62.49} & 69.19 & \bluecellnp{70}{43.32} & \bluecellnp{70}{58.33} \\

DF2K~\cite{df2k1,df2k2,df2k3,df2k4}       
& 45.99 & 52.92 & 34.78 & 44.56 \\

LAION-5B~\cite{laion5b}   
& 60.56 & \bluecellnp{70}{69.21} & 38.85 & 56.21 \\

\midrule
\multicolumn{5}{l}{\textit{\textbf{AIGC Images}}} \\
Blip3o-60K~\cite{chen2025blip3ofamilyfullyopen} 
& \bluecellnp{100}{63.81} & \bluecellnp{100}{73.88} & \bluecellnp{100}{49.38} & \bluecellnp{100}{62.36} \\

ImgEdit~\cite{ye2025imgeditunifiedimageediting}    
& 55.83 & 59.77 & 36.88 & 50.83 \\

\bottomrule[1.5pt]
\end{tabular}

\end{threeparttable}}
\vspace{-15pt}
\end{table}


% \vspace{-10pt}
% \subsubsection{Application}
% \label{sec:application_unipercept}

% The perceptual-level understanding capability of UniPercept enables a broad range of downstream applications. A primary use case is employing its multi-dimensional visual rating ability—spanning \textit{Aesthetics Quality} (IAA), \textit{Image Quality} (IQA), and \textit{Structure \& Texture Richness} (ISTA)—as a \textbf{reward model} for text-to-image generation. We integrate all these ratings as reward into the Flow-GRPO~\cite{liu2025flowgrpotrainingflowmatching} fine-tuning pipeline based on FLUX.1-dev~\cite{flux}. The results in Tab.~\ref{tab:application} and Fig.~\ref{fig:application_result} show that incorporating UniPercept reward leads to clear improvements in human preference, quality, and aesthetics metrics, substantially enhancing the perceptual quality of the generated images. UniPercept can also serve as a unified set of \textbf{perceptual metrics} for evaluating generated images, as reflected in the quantitative results in Tab.~\ref{tab:application}. More applications are provided in Appendix.

% \begin{table}[htbp]
% % \vspace{-10pt}
% \centering
% \small
% \setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{0.9}
% \caption{\textbf{Performance of FLUX.1-dev w/ UniPercept Reward.}}
% % \vspace{-8pt}

% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{l cc c cc ccc}
% \toprule
% \multirow{2}{*}{\textbf{Models}} &
% \multicolumn{2}{c}{\textbf{Preference Score}} &
% \multicolumn{1}{c}{\textbf{Image Quality}} &
% \multicolumn{2}{c}{\textbf{Image Aesthetics}} &
% \multicolumn{3}{c}{\textbf{UniPercept Score}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-4}
% \cmidrule(lr){5-6} \cmidrule(lr){7-9}
% & PickScore~\cite{pickscore} & HPSv3~\cite{hspv3} & DeQA~\cite{deqa_score} & LAION-Aes~\cite{laion-aes} & ArtiMuse~\cite{artimuse} & IAA & IQA & ISTA \\
% \midrule
% Baseline & 22.46 & 10.71 & 4.32 & 5.77  & 59.02 & 65.18 & 73.59 & 46.64 \\
% \textbf{w/ UniPercept Reward} 
% & \textbf{\bluecellnp{100}{22.67}} 
% & \textbf{\bluecellnp{100}{10.93}} 
% & \textbf{\bluecellnp{100}{4.33}} 
% & \textbf{\bluecellnp{100}{6.19}} 
% & \textbf{\bluecellnp{100}{65.52}} 
% & \textbf{\bluecellnp{100}{74.24}} 
% & \textbf{\bluecellnp{100}{77.04}} 
% & \textbf{\bluecellnp{100}{59.08}} \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:application}
% % \vspace{-12pt}
% \end{table}

% \begin{figure}[htbp]
%     % \vspace{-10pt}
%     \centering
%     \includegraphics[width=0.45\textwidth]{unipercept/Figures/exp/application_v1.pdf}
%     \vspace{-5pt}
%     % \caption{\textbf{Results of FLUX.1-dev with UniPercept reward.} 
%     % The scores are generated by UniPercept across \textcolor{RubineRed}{IAA}/\textcolor{blue}{IQA}/\textcolor{Mulberry}{ISTA}.}
%     \caption{\textbf{Results of FLUX.1-dev w/ UniPercept Reward.}}
%     % \caption{\textbf{Quantitative results of UniPercept reward}.}
%     \label{fig:application_result}
%     % \vspace{-20pt}
% \end{figure}


\section{Conclusion}
\label{sec:Conclusion}
% \vspace{-5pt}


We provide \textbf{UniPercept-Bench}, a unified benchmark built on a hierarchical definition for perceptual-level image understanding. 
We also develop a strong baseline \textbf{UniPercept} through Domain-Adaptive Pre-training and Task-Aligned RL, which generalizes well across perceptual domains and outperforms existing MLLMs. 
UniPercept further serves as a plug-and-play \textbf{reward model} for perceptually aligned post-training of T2I models, enabling controllable improvements in perceptual attributes. Beyond model optimization, it also offers a unified perceptual diagnostic tool that reveals systematic behavioral and dataset-level patterns, highlighting its broader utility for future perceptual-level research.


\noindent\textbf{Limitations.}
Although UniPercept-Bench is sufficiently large for current perceptual-level tasks, it remains smaller than typical semantic-level benchmarks. Further expansion in scale will be explored in future work.
